Constraining the low-energy S=-2 meson-baryon interaction with two-particle correlations

The two-particle correlation technique applied to $K^-\Lambda$ pairs in pp collisions at LHC recently provided the most precise data on the strangeness $S=-2$ meson-baryon interaction. In this letter, we use for the first time femtoscopic data to constrain the parameters of a low-energy effective QCD Lagrangian. The tuned model delivers new insights on the molecular nature of the $\Xi(1620)$ and $\Xi(1690)$ states. This procedure opens the possibility to determine higher order corrections, directly constraining QCD effective models particularly in the multi-strange and charm sectors.

==> sections/UntrimmedVersion/Correlation_Fitting.tex <==
\textit{Fitting procedure:} In our study we focus on the \LKMin correlation function recently measured by ALICE in \pp collisions~\cite{LKALICEpp}. Following the approach in~\cite{LKALICEpp}, the total function we use to fit the data reads

\begin{align}\label{eq:totcorrelation}
    C_\mathrm{tot}(\kstar) = & N_D \times C_\mathrm{model}(\kstar) \times C_\mathrm{background} (\kstar).
\end{align}
The term $C_\mathrm{model}(\kstar)=1 + \lambda_{\rm gen.} \times (C_{\rm gen.}(\kstar) - 1)+ \sum_{i} \lambda_{i} \times (C_{i}(\kstar) - 1)$ includes the genuine \LKMin correlation, defined via Eq.~(\ref{eq:corrfun_CC}) and depending on the parameters of the VBC model, as well as the residual contributions, consisting mainly of primary kaons and secondaries \lmb, stemming from the weak decays of charged and neutral $\Xi$ and from the electromagnetic decay of $\Sigma^0$ ($i=\Xi^{0,-}K^-,\Sigma^0 K^-$). Both the genuine and residual correlations are weighted with the same \lmb parameters obtained in~\cite{LKALICEpp} (e.g. $\lambda_{\mathrm{gen}}=51\%$). The interaction amongst the pairs composing the residual correlations are modeled using the same assumptions adopted in~\cite{LKALICEpp}.\\
{\color{purple} \bf This next paragraph on the sources is a little bit messy and long. Can it be rewritten?}
A prior knowledge of the source function is needed in general to evaluate both the genuine and residual contributions~\cite{femtoreview,LisaPrattReview}. 
In particular, to obtain the $C_{\rm gen.}(\kstar)$ correlation for the \LKMin system from Eq.~\ref{eq:corrfun_CC}, we determined the specific emitting sources for each elastic (\LKMin) and inelastic (\PiMinXiZ, \PiZXiMin, \KMinSigZ, \KZbarSigMin and \EtaXiMin) channel, following the same approach used in the treatment of the coupled-channel contributions in the analysis of the \kMinProt correlation in~\cite{ALICE:pKCoupled}. For the elastic contribution ($j=i=\LKMin$), we assumed the same double Gaussian parametrization for the source employed in~\cite{LKALICEpp}. Values of the parameters and its uncertainties are reported in~~\cite{LKALICEpp}. For the elastic source part, the radii for the two gaussians are of the order of $1.2$ fm and $2.3$ fm, respectively. The same values and source distribution is assumed also for the residual correlations.\\
As shown in~\cite{ALICE:pKCoupled}, depending on the pairs entering the inelastic contributions, the corresponding source profiles can significantly deviates from the elastic one. Such an effect is particularly relevant when pions are involved, as in the case at hand here in which the channels \PiMinXiZ and \PiZXiMin are present. We performed a detailed study on the source profiles of these and the remaining inelastic channels by adopting the data-driven resonance source model (RSM) in~\cite{ALICE:Source}, used as well in the \LKMin correlation measurement~\cite{LKALICEpp} and in several femtoscopic analyses~\cite{ALICE:pOmega,ALICE:LXi,ALICE:BBar,ALICE:pLCoupled,ALICE:pXi,ALICE,ALICE:pD}, including the recent one on the \kMinProt coupled-channel dynamics in~\cite{ALICE:pKCoupled}. 
Following the RSM prescriptions and the work in~\cite{ALICE:pKCoupled}, we build a gaussian core source, common to all inelastic channel, with the reported radius of $r_\mathrm{core}=1.11\pm0.04$ in~\cite{LKALICEpp}. The non-gaussian contributions to this common source part are specific for each channel we are considering (\PiMinXiZ, \PiZXiMin, \KMinSigZ, \KZbarSigMin and \EtaXiMin) since they involve the feeding from strongly decaying resonances. By adopting the same procedure described in details in~\cite{ALICE:pKCoupled}, we estimated the kinematics and yield production of each inelastic pair in the high-multiplicity \pp data sample using available transport~\cite{EPOSLHC} and thermal models~\cite{TFMultiplicity}. As done for the elastic \LKMin channel, the final inelastic sources, composed of the common core and the resonance contributions, can be then modeled with a double gaussian parametrization. Compatible values of parameters are found between the \KMinSigZ and \KZbarSigMin effective sources and the \LKMin one, while larger radii ($R_1\approx 1.4$ fm, $R_2\approx3.3$ fm) are obtained for the $\uppi\Xi$ channels due to the long-lived resonances ($c\tau \gtrsim 5$ fm) feeding to the pions. The remaining $S_{\EtaXiMin}(\rstar)$ distribution, since no significant strong feed-down to the $\Xi$ baryon is present, is localized at slightly smaller \rstar ($R_1\approx 1.2$ fm, $R_2\approx2.2$ fm).
We assigned the same relative uncertainties on the inelastic source´s parameters using the reported one ($\approx4\%$) on the $r_{\mathrm{core}}$ in~\cite{LKALICEpp}.
Values and additional details on the determination of the emitting source can be found in the Supplemental material.\\
The fit of the VBC model to the measured \LKMin correlation requires a proper determination of the production weights $\omega_{j} ^{\rm prod.}$ in Eq.~(\ref{eq:corrfun_CC}). The estimate of these weights is determined in a data-driven approach following the same method adopted in the $K^- - p$ correlation analysis for the same high-multiplicity dataset~\cite{ALICE:pKCoupled}. The yields of the pairs in each $j$ channel are obtained assuming a thermal production~\cite{Thermalfist} and the corresponding \kstar distribution are derived by using as input the Blast-wave parametrization of the measured transverse momentum spectra of the single particles in the pair.
%At first, the yields of pairs in each $j$ channel are estimated within a thermal approach using the public THERMAL-FIST (TF) framework~\cite{Thermalfist}. The values, and the corresponding uncertainties, for the input TF parameters (e.g temperature $T$) are obtained from the parameterisation provided in Ref.~\cite{TFMultiplicity} at the average multiplicity of charged particles at mid-rapidity $\langle \dndeta \rangle = 31.6$~\cite{ALICE:pOmega} in the considered \pP dataset used for the measurement of \LKMin correlations~\cite{LKALICEpp}. Next, we estimate the \kstar distribution of each channel using as input the transverse momenta spectra \pt of the single particles in the pair. The latter is obtained using a Blast-wave (BW) fit approach using the same parameters as in~\cite{ALICE:pKCoupled} for the high-multiplicity \pP collisions dataset. Based on the BW spectra, the \kstar distribution for the pairs is built, selecting only relative momenta in the femtoscopic region $\kstar < 200 \MeVc$.
%To obtain the final production weights, the integrated BW pair yield in the considered \kstar range is rescaled by the corresponding pair yield evaluated within TF and normalized to the \LKMin one, taken as a reference.
The values obtained for each inelastic channel (normalized to the \LKMin one, e.g. $\omega_{\LKMin} ^{\rm prod.} = 1.$) are $\omega_{\PiMinXiZ} ^{\rm prod.} = 1.53$, $\omega_{\PiZXiMin} ^{\rm prod.} = 1.58$, $\omega_{\KMinSigZ} ^{\rm prod.} = 0.68$, $\omega_{\KZbarSigMin} ^{\rm prod.} = 0.63$ and $\omega_{\EtaXiMin} ^{\rm prod.} = 0.18$. 
We associated errors on the productions weights of the order of maximum $\approx10\%$ by propagating the available uncertainties on the parameters used to estimate the yields of the inelastic pairs~\cite{TFMultiplicity} and its \kstar kinematics, as done in~\cite{ALICE:pKCoupled}. Additional informations can be found in the Supplemental Material.\\
For the comparison with the measured \LKMin correlation in~\cite{LKALICEpp}, a residual background, given by the last term in Eq.~(\ref{eq:corrfun_CC}), must be taken into account. 
The profile of $C_\mathrm{background} (\kstar)$, publicly available at~\cite{hepdata.143518}, includes the presence of several resonances and in particular the \XResNovanta. In~\cite{LKALICEpp}, the \XResNovanta has been modeled with a Breit-Wigner distribution and the corresponding mass and widths extracted from the fit were found compatible with the PDG values~\cite{PDG}. In our work, the \XResNovanta is dynamically generated within the VBC model in the $C_\mathrm{model} (\kstar)$ term, hence the region in \kstar of the background associated to this state should be removed. We performed a fit to the available $C_\mathrm{background} (\kstar)$, using Eq.~(3) in~\cite{LKALICEpp}, and we set to zero the corresponding Breit-Wigner term for the \XResNovanta. With this procedure, the final background correlation entering in our fit in Eq.~(\ref{eq:totcorrelation}) only contains as resonances the weakly decaying $\Omega$ at $\kstar \approx 210$ \MeVc and the \XResVenti at $\kstar \approx 400$ \MeVc.\\
%add momentum smearing info and residual momentum matrix
The fit of the total correlation in Eq.~(\ref{eq:totcorrelation}) to the \LKMin correlation data is performed, following~\cite{LKALICEpp}, in the range $0 \leq \kstar \leq 500$ \MeVc, leaving as free parameters the normalization constant $N_D$ and the LECs and subtraction constants $a_i$ of the VBC model.
The fitting procedure we adopt is based on the bootstrap technique used as well in~\cite{LKALICEpp}, in order to properly include the statistical and systematic uncertainties of the data. A total of 1000 samplings is performed in which we also, at each iteration, random vary the sources parameters and production weights values within the quoted uncertainties.\\


==> sections/UntrimmedVersion/Correlation_Formalism.tex <==
\newline
\textit{Formalism:} %In the presence of a two-particle system, whose interaction is characterized by the presence of several $j$ coupled channels, the corresponding correlation function reads~\cite{LisaPrattReview,Haidenbauer:CC,Kamiya:CCKp}
{\color{red}In the case of a multi-channel system, such as the one we are dealing with in this work, the corresponding two-particle correlation function of a given observed channel $i$ reads~\cite{LisaPrattReview,Haidenbauer:CC,Kamiya:CCKp}}

\begin{align}\label{eq:corrfun_CC}
    C_i(\ks) = \sum_{j} \omega_{j} ^{\rm prod.} \int d^3 \rstar S_{j} (\rstar) |\psi_{ji} (\ks,r^*)|^2.
\end{align}

Here \kstar and \rstar represent, respectively, the relative momentum and distance between the two particles, measured in the pair rest frame. 
The contributions of the $j$ channels  are scaled by the production weights $\omega_{j} ^{\rm prod.}$, which take into account the abundance of pairs produced as initial states in each coupled channel. The function $S_{j}(\rstar)$ is the so-called emitting source, which particularly in small colliding system, can be different in each channel depending on the feed-down from strong resonances (with a lifetime $\approx 1-2$ fm/c) to the pair we are considering~\cite{ALICE:Source,ALICE:pKCoupled,CECA}. The last ingredient is the relative wave function $\psi_{ji} (\ks,r^*)$, which embeds the strong interaction arising from the coupled-channel dynamics in the system {\color{red}, and it can be obtained from the scattering amplitude $T$ as
\begin{widetext}
\begin{equation}
\Psi_{ji}(\ks,r^*) = \delta_{ji} j_0(\ks r^*)
+\int d^3q^* \frac{j_0(q^*r^*)T_{ji}(E, \ks,q^*)
}{E-E_1^{(j)}(q^*)-E_2^{(j)}(q^*)+i\,\eta} \ ,
\label{eq:WF}
\end{equation}
\end{widetext}
where $E_1^{(j)}(q^*)$ and $E_2^{(j)}(q^*)$ are the relativistic kinetic energies of particles $1$ and $2$ in channel $j$, $E=E_1^{(i)}(\ks)+E_2^{(i)}(\ks)$ is the total energy of the observed channel $i$ in their center-of-mass frame, and the scattering amplitude $T_{ji}(E, \ks,q^*)$ is obtained by using an on-shell factorization of the Bethe--Salpeter equation with an ultraviolet regularized separable $s$-wave potential which leads to a scattering amplitude of the form
\begin{equation}
T_{ji}(E,\ks,q^*) = T_{ji}(E)\theta(q_{max}-\ks)\theta(q_{max}-q^*) \ ,
\label{eq:Tmat}
\end{equation}
where the cut-off momentum $q_{max}$ is taken in this work equal to 850 MeV/c.} 
We define for simplicity $i=j=1$ as the elastic \LKMin channel, namely the pair measured experimentally, and $j\neq 1$ indicates the remaining inelastic \XiPi-\LAK-\SIK-\XiEta channels.

\textcolor{blue}{ The procedure to obtain the scattering amplitudes within the UChPT scheme departs from the chiral effective Lagrangian, up to NLO in this case, given by
$
\mathcal{L}_{\phi B}^{eff}=\mathcal{L}_{\phi B}^{(1)}+\mathcal{L}_{\phi B}^{(2)}  \ ,
$
with
%
\begin{eqnarray} 
\mathcal{L}_{\phi B}^{(1)} & = & i \langle \bar{B} \gamma_{\mu} [D^{\mu},B] \rangle
                            - M_0 \langle \bar{B}B \rangle  
                           - \frac{1}{2} D \langle \bar{B} \gamma_{\mu} 
                             \gamma_5 \{u^{\mu},B\} \rangle \nonumber \\
                  & &      - \frac{1}{2} F \langle \bar{B} \gamma_{\mu} 
                               \gamma_5 [u^{\mu},B] \rangle \ ,
\label{LagrphiB1} 
\end{eqnarray} 
\begin{eqnarray} 
  \mathcal{L}_{\phi B}^{(2)}& = & b_D \langle \bar{B} \{\chi_+,B\} \rangle
                             + b_F \langle \bar{B} [\chi_+,B] \rangle
                             + b_0 \langle \bar{B} B \rangle \langle \chi_+ \rangle  \nonumber \\ 
                     &  & + d_1 \langle \bar{B} \{u_{\mu},[u^{\mu},B]\} \rangle 
                            + d_2 \langle \bar{B} [u_{\mu},[u^{\mu},B]] \rangle     \nonumber \\
                    &  &  + d_3 \langle \bar{B} u_{\mu} \rangle \langle u^{\mu} B \rangle
                            + d_4 \langle \bar{B} B \rangle \langle u^{\mu} u_{\mu} \rangle \ .
\label{LagrphiB2}
\end{eqnarray}
In these equations, $B$ is the octet baryon matrix, while the matrix of the pseudoscalar mesons $\phi$  is implicitly contained in 
$u_\mu = i u^\dagger \partial_\mu U u^\dagger$, where $U(\phi) = u^2(\phi) = \exp{\left( \sqrt{2} {\rm i} \phi/f \right)} $ with $f$ being the meson decay constant. 
The covariant derivative is given by  $[D_\mu, B] = \partial_\mu B + [ \Gamma_\mu, B]$, with $\Gamma_\mu =  [ u^\dagger,  \partial_\mu u] /2$, while $\chi_+ = 2 B_0 (u^\dagger \mathcal{M} u^\dagger + u \mathcal{M})$, with $\mathcal{M} = {\rm diag}(m_u, m_d, m_s)$ and $B_0 = - \langle 0 |\bar{q} q | 0 \rangle / f^2$, is the explicit chiral symmetry breaking term. The values of the axial vector constants are taken as $D=0.8$ and $F=0.46$, fulfilling the $g_A=D+F=1.26$ constraint,  and $M_0$ is the baryon octet mass in the chiral limit. The NLO Lagrangian depends on a few LECs, namely $b_D$, $b_F$, $b_0$ and $d_i$ $(i=1,\dots,4)$, to be determined from experiment since they are not constrained by the symmetries of the theory. }\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht]
\begin{center}
\centering
\includegraphics[width=3.4 in]{Figures/Diagrams.pdf}% Here is how to import EPS art
\vspace{-0.4cm}
\caption{Feynman diagrams for meson-baryon interaction: WT term (i), direct and crossed Born terms (ii) and (iii), and NLO terms (iv). Dashed (solid) lines represent the pseudoscalar octet mesons (octet baryons).}
\label{fig:diagrams} 
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textcolor{blue}{Next step consists of deriving the meson-baryon interaction kernel in momentum space from Eqs.~(\ref{LagrphiB1}) and (\ref{LagrphiB2}).
 Specifically, by inspecting Fig~\ref{fig:diagrams}, the contact diagram (i) corresponds to the the Weinberg-Tomozawa (WT) contribution that comes from the covariant derivative in Eq.~(\ref{LagrphiB1}). The vertices of direct (diagram (ii)) and crossed Born (diagram (iii)) contributions are obtained from the second and third term in Eq.~(\ref{LagrphiB1}); while the tree-level NLO contributions are fully extracted from (\ref{LagrphiB2}) whose schematically representation is shown by the fourth diagram of  Fig.~\ref{fig:diagrams}. Thus, the total interaction kernel up to NLO considered in this work can be expressed as the sum:
$
%\begin{equation}
%\label{V_TOT}
 V_{ij}=V^{\scriptscriptstyle WT}_{ij}+V^{D}_{ij}+V^{C}_{ij}+V^{\scriptscriptstyle NLO}_{ij} ,
%\end{equation}
$
where the elements of the $\hat{V}_{ij}$ interaction matrix couple all possible meson-baryon channels ($\pi^0\Xi^-$, $\pi^-\Xi^0$, $K^-\Lambda$, $K^-\Sigma^0$, $\bar{K}^0 \Sigma^-$, $\eta\Xi^-$).
The reader is referred to \cite{Feijoo:2021zau}, Eqs.~(7)-(10), for the general structure of the different contributions to the final interaction kernel. However, considering that we limit the model to the s-wave projection the final expressions for the kernels are those of Eqs.~(6)-(8) and (10) in Ref.~\cite{Ramos:2016odk}. The dynamical bulk in the former expressions is preceded by the corresponding $C_{ij}$ coefficients that encode the symmetries of the interaction. In the case of the NLO contribution, particularly called $L_{ij}$ and $D_{ij}$ in \cite{Ramos:2016odk}, they come in terms of linear combinations of the LECs present in Eq.\ (\ref{LagrphiB2}). At this point, we need to employ basic isospin arguments to construct the interaction kernel in the ($S=-2,\,Q=-1$) sector from the ($S=-2,\,Q=0$) one whose machinery was developed in \cite{Feijoo:2023wua}.
The presence of $\Xi^*$ resonances prevents the use of a plain Chiral Perturbation Theory (ChPT) expansion, thus making nonperturbative treatment mandatory. The UChPT method consists of solving the Bethe-Salpeter equations that can be done through an on-shell factorization leaving a simple system of algebraic equations expressed in matrix form as:
%
\begin{equation}
T_{ij} ={(1-V_{il}G_l)}^{-1}V_{lj} ,
 \label{T_algebraic}
\end{equation}
% 
where $T_{ij}$ is scattering amplitude for a given starting i-channel and an outgoing j-channel, and $G_l$ is the loop function standing for a diagonal matrix. Since this function diverges logarithmically, the dimensional regularization is applied obtaining as final expression:
%
\begin{eqnarray}
 G_l & = &\frac{2M_l}{(4\pi)^2} \Bigg \lbrace a_l(\mu)+\ln\frac{M_l^2}{\mu^2}+\frac{m_l^2-M_l^2+s}{2s}\ln\frac{m_l^2}{M_l^2}  \nonumber \\ 
 &  +   &  \frac{q_{\rm cm}}{\sqrt{s}}\ln\left[\frac{(s+2\sqrt{s}q_{\rm cm})^2-(M_l^2-m_l^2)^2}{(s-2\sqrt{s}q_{\rm cm})^2-(M_l^2-m_l^2)^2}\right]\Bigg \rbrace .  
 \label{dim_reg}    
\end{eqnarray}
%
The loop function $G_l$ comes in terms of the baryon ($M_l$) and meson ($m_l$) masses for the $l$-channel as well as the subtraction constants (s.c.) $a_l$ that replace the divergence for a given dimensional regularization scale $\mu$ which is taken to be $1$~GeV. Despite a natural size can be established for them, the lack of knowledge about the $a_l$ constants implies the inclusion of them in fitting procedures to be determined. The number of independent s.c. is reduced by isospin symmetry arguments which, in this case, amount to four. 
Summarizing, the UChPT scheme taking into account WT+Born+NLO terms in this sector leaves a scattering amplitude that depends on $13$ parameters never determined before. The $\Lambda K^-$ correlation function offers an unprecedented opportunity to consolidate a theoretical model that can be employed to make novel predictions in a quite unknown sector.} \\
The approach to fit the LECs and subtraction constants of {\color{red}this model, referred from now on as the Valencia--Barcelona--Catania (VBC) model}, is described in the following section.\\


==> sections/UntrimmedVersion/Introduction.tex <==
%\section{Introduction} \label{sec:intro}
\textit{Introduction:} The dynamics of the strong interaction between strange hadrons at low {\color{red} and intermediate} energies is still a rather uncharted territory, both %on the experimental side and, consequently, also on the theoretical side. 
{\color{red} experimentally and theoretically.}
Effective Lagrangians {\color{red} in terms of hadronic degrees of freedom}, including the fundamental symmetries of Quantum-Chromo-Dynamics (QCD), are widely used %in this non-perturbative regime to model the exact QCD force in a limited energy range, typically below the nucleon mass.\\
{\color{red} to circumvent the mathematical problems raised by the non-perturbative character of QCD at low and intermediate energies which makes still difficult a fully quantitative description of the hadron-hadron interactions in terms of the underlying quark and gluon dynamics.}
{\color{purple} {\bf Alternative text for the previous sentence:} A fully quantitative description of hadron interactions in terms of the elementary quark and gluon degrees of freedom is hindered by the mathematical problems associated to the non-perturbative character of Quantum-Chromo-Dynamics (QCD) at low and intermediate energies. Effective Lagrangians, employing hadronic degrees of freedom and including the fundamental symmetries of QCD, are widely used to circumvent this difficulty. }\\
Amongst these effective approaches, Chiral Perturbation theory (ChPT) scheme {\color{red} has} proved to be an extremely powerful tool \sout{to compute in a systematic way many low-energy observables (e.g cross-sections) and to provide insights on the underlying hadronic interactions. The ChPT framework allows us to investigate higher-orders terms in the chiral expansion of the interaction, which, in principle, can significantly improve the understanding of the underlying QCD dynamics in the system at hand.} {\color{purple} {\bf I do  not like the word ``compute" here. My proposal is:}, allowing for a systematic implementation of higher order terms of the chiral expansion, which can in principle significantly improve the understanding of the QCD dynamics of the system at hand.} 
 Each \sout{interaction} term in the Lagrangian is \sout{weighted} preceded by the so-called Low Energy Constants (LECs), parameters which are not fixed by the underlying theory and hence must be determined by a fit to the available %measurements.
{\color{red} experimental data.}\\ 
%The unstable nature of strange baryons ($\lmb$, $\Sigma$, $\Xi$, $\Omega$ and corresponding anti-particles),  makes extremely challenging to perform scattering experiments and, hence it significantly reduces the amount of data available on the strong interaction of hyperons with strange mesons, such as kaons ($K$) and antikaons ($\overline{K}$).
In this work we are interested in the $S=-2$ meson-baryon sector, dominated by the \XiPi-\LAK-\SIK-\XiEta coupled-channel dynamics. Current experimental information includes only the evidence of the excited \XResNovanta resonance decaying into \LKMin, reported by LHCb and Belle~\cite{LHCb,BELLE} and the first observation by Belle of the neutral \XRes decaying into $\Xi^-\uppi^+$~\cite{BELLE}. \sout{The scarce amount of data is not sufficient to constrain all the LECs and possible additional parameters of the available effective models and eventually these input are fixed via $SU(3)$ flavour symmetry considerations or by using the larger data sample available on the \kbarN interaction in the $S=-1$ sector~\cite{Humphrey:1962zz,Watson:1963zz,Mast:1975pv,Nowak:1978au,Ciborowski:1982et,Sakitt:1965kh,Bazzi11,Bazzi12,Lambda1405_1,Lambda1405_2,Lambda1405_3,Lambda1405_4,Lambda1405_CLAS}.} {\color{purple} {\bf I modified the previous sentence into this one: } This scarce amount of data is not sufficient to constrain the next-to-leading order LECs of the $S=-2$ effective model. The strategy in ~\cite{Feijoo:2023wua} has been to invoke $SU(3)$ flavour symmetry arguments to adopt the same LECs as those of the \kbarN interaction models in the $S=-1$ sector, which benefit from a much larger data sample~\cite{Humphrey:1962zz,Watson:1963zz,Mast:1975pv,Nowak:1978au,Ciborowski:1982et,Sakitt:1965kh,Bazzi11,Bazzi12,Lambda1405_1,Lambda1405_2,Lambda1405_3,Lambda1405_4,Lambda1405_CLAS}.}
Similarly to the $\Lambda(1405)$, a molecular \SPi-\kbarN state arising from the interplay between these two coupled-channels, the \XRes and \XResNovanta resonances might also be generated within the \XiPi-\LAK-\SIK-\XiEta dynamics, thereby acquiring a molecular structure.


A large theoretical effort was devoted in  the last two decades~\cite{Ramos02,Garcia-Recio1,Garcia-Recio2,Sekihara:2015qqa,Khemchandani:2016ftn,Nishibuchi:2023acl} to the understanding of the nature and properties of the \XRes and \XResNovanta
states but the community is still missing a clear picture on the corresponding values of masses and widths. Recently, the authors in~\cite{Feijoo:2023wua} delivered the first  effective meson-baryon Lagrangian, obtained within the  UChPT framework, that includes contributions beyond the leading contact-term only interaction.
The introduction of higher-orders in the chiral expansion is needed to reduce the disagreemnt between models and the available measurements of the two $\Xi^{\ast}$ states but it also comes at the expenses of introducing more LECs, namely more unknown parameters to be constrained from data. Hence, the improvement in the theoretical developments on the $S=-2$ meson-baryon interaction achieved in these latest calculations must be followed by the addition of more high-precision experimental data.

{\color{purple}{\bf And yet another proposal of the whole previous paragraph:} 
In this work we are interested in the $S=-2$ meson-baryon sector, dominated by the \XiPi-\LAK-\SIK-\XiEta coupled-channel dynamics. Similarly to the $\Lambda(1405)$, a molecular \SPi-\kbarN state arising from the interplay between these two coupled-channels \cite{} (CITE a few overview papers here), the \XRes and \XResNovanta resonances might also be dynamically generated from the coupled-channel $S=-2$ meson-baryon interaction, thereby acquiring a molecular structure. A large theoretical effort was devoted in  the last two decades~\cite{Ramos02,Garcia-Recio1,Garcia-Recio2,Sekihara:2015qqa,Khemchandani:2016ftn,Nishibuchi:2023acl} to the understanding of the nature and properties of the \XRes and \XResNovanta
states but the community is still missing a clear picture on the corresponding values of masses and widths. Recently, the authors in~\cite{Feijoo:2023wua} delivered the first  effective meson-baryon Lagrangian\sout{, obtained within the  UChPT framework,} that includes contributions beyond the leading contact-term interaction.
The introduction of higher-orders in the chiral expansion is needed to reduce the disagreemnt between models and the available measurements of the two $\Xi^{\ast}$ states but it also comes at the expense of introducing more LECs, namely more unknown parameters, to be constrained from data. Unfortunatelly, current experimental information includes only the evidence of the excited \XResNovanta resonance decaying into \LKMin, reported by LHCb and Belle~\cite{LHCb,BELLE} and the first observation by Belle of the neutral \XRes decaying into $\Xi^-\uppi^+$~\cite{BELLE}. This scarce amount of data is not sufficient to constrain the next-to-leading order LECs of the $S=-2$ effective model \cite{Feijoo:2023wua} and $SU(3)$ flavour symmetry arguments were invoked to adopt the same LECs as those of the \kbarN interaction models in the $S=-1$ sector, which benefit from a much larger data sample~\cite{Humphrey:1962zz,Watson:1963zz,Mast:1975pv,Nowak:1978au,Ciborowski:1982et,Sakitt:1965kh,Bazzi11,Bazzi12,Lambda1405_1,Lambda1405_2,Lambda1405_3,Lambda1405_4,Lambda1405_CLAS}. Hence, the improvement in the theoretical developments on the $S=-2$ meson-baryon interaction requires the availability of more high-precision experimental data.}

%A pivotal work on the $S=-2$ meson-baryon interaction within a $SU(3)$ Unitarized ChPT (UChPT) approach, well before the Belle´s results became available, demonstrated for the first time the existence of a  pole located roughly 5 MeV below the \LAK threshold, assigned to the \XRes and clearly different from the \XResNovanta state~\cite{Ramos02}. Similar studies were performed after this, which qualitatively provided a consistent picture of both $\Xi^{\ast}$ states, but they failed at delivering a common picture on the values of masses and widths of the corresponding poles~\cite{Garcia-Recio1,Garcia-Recio2,Sekihara:2015qqa}.
%A recent new work~\cite{Nishibuchi:2023acl}, based on the same approach as in~\cite{Ramos02}, included the experimental information from Belle and delivered a description of the \XRes state compatible with the data. However, the input parameters of the model had to be significantly reduced, beyond their expected natural range, to achieve such an agreement. Still within the UChPT framework, an extension beyond the leading contact-term only interaction assumed in ~\cite{Ramos02} has been recently published~\cite{Feijoo:2023wua}. The authors in~\cite{Feijoo:2023wua} showed that the inclusion of Born and next-to-leading-order contributions in the lagrangian is needed in order to improve the agreement of the model with the measured properties of the \XRes and \XResNovanta. 
%The introduction of higher-orders in the chiral expansion comes at the expenses of introducing more LECs, namely more unknown parameters to be constrained from data. In absence of enough experimental data in this sector, the authors in~\cite{Feijoo:2023wua} anchored the parameters of the model to the available \kbarN $S=-1$ measurements. Such symmetry assumption, even if required to calculate the physics observables, might not be fully valid and it could be at the origin of a tension in reproducing the width of both \XRes and \XResNovanta in~\cite{Feijoo:2023wua}.  
%The take-home message from these first two decades of dedicated theoretical efforts in the description of the $S=-2$ meson-baryon interaction is that more high-precision and differential data are needed if we want to quantitatively constrain the model´s parameters and improve our understanding on the nature of the \XRes and \XResNovanta state.\\ 
Such experimental input became available with the recent measurement of the \LKMin correlation in the high-multiplicity \pp sample at \onethree by the ALICE collaboration delivering the most precise data on this interaction and providing the first experimental observation of the \XRes decaying into \LKMin pairs~\cite{LKALICEpp}. These data rely on the femtoscopy technique applied at LHC in \pp collisions~\cite{femtoreview} which
%in which the relative distances of the particles in the pair are roughly 1-2 fm and hence the measured correlation not only shows a large sensitivity to the strong potential but also to the short-range coupled-channel dynamics. This approach 
already proved to grant, with an unprecedented precision, the experimental access to a large amount of interactions involving strange and charm hadrons~\cite{ALICE:Run1,ALICE:pXi,ALICE:pSig0,ALICE:LL,ALICE:pOmega,ALICE:pKpp,ALICE:pKCoupled,ALICE:pLCoupled,ALICE:BBar,ALICE:LXi}.\\
%ALICE:Run1,ALICE:pXi,ALICE:pSig0,ALICE:pOmega,ALICE:LL,ALICE:pKpp,ALICE:pKCoupled,ALICE:pLCoupled,ALICE:BBar,ALICE:LXi
%Baryon-baryon potentials, for heavy systems as N$\Xi$ and N$\Omega$, obtained from lattice QCD calculations at the physical quark masses CITE HAL QCD were tested on the measured correlation functions for the first time, opening the possibility to validate predictions based on the exact QCD lagrangian. Interacting potentials for lighter systems, such as the \LAK investigated in this work, cannot be determined on the lattice with the same accuracy  and, hence a particular effort should be devoted to constraining the state-of-the-art ChPT models.
%The measured \LKMin correlation in the high-multiplicity \pp sample at \onethree recently published by the ALICE collaboration CITE ALICE delivered the most precise data on this interaction and provided the first experimental observation of the \XRes decaying into \LKMin pairs. 
In the present Letter we use for the first time femtoscopic data on the \LKMin pairs measured by the ALICE Collaboration in \pp collisions~\cite{LKALICEpp} to fit the parameters of the state-of-the-art UChPT effective Lagrangian at next-to-leading-order (NLO)~\cite{Feijoo:2023wua}. 
The extracted LECs and parameters are used to investigate the position and couplings to the different channels of the poles related to the \XRes and \XResNovanta states, leading to a complete new scenario for the molecular composition of the \XRes resonance.\\ 
The results presented in this work pave the way for a novel method to constrain the low-energy QCD effective models for interactions involving multi-strange and charm hadrons, which cannot be accessed via traditional scattering experiments. For these interactions, correlation measurements at LHC~\cite{ALICERun3Run4,ALICE3} will be in the near future the only experimental data available for constraining models, hence the methodology described in this Letter provide a tool to constrain the QCD dynamics in the non-perturbative regime.
